Chrion: Optimizing Recurrent Neural Network Inference by Collaboratively Utilizing CPUs and GPUs

Deploying deep learning models in cloud clusters provides efficient and prompt inference services to accommodate the widespread application of deep learning. These clusters are usually equipped with host CPUs and accelerators with distinct responsibilities to handle serving requests, i.e. generalpurpose CPUs for input preprocessing and domain-specific GPUs for forward computation. Recurrent neural networks play an essential role in handling temporal inputs and display distinctive computation characteristics because of their high inter-operator parallelism. Hence, we propose Chrion to optimize recurrent neural network inference by collaboratively utilizing CPUs and GPUs. We formulate the model deployment in the CPU-GPU cluster as an NP-hard scheduling problem of directed acyclic graphs on heterogeneous devices. Given an input model in the ONNX format and user-defined SLO requirement, Chrion firstly preprocesses the model by model parsing and profiling, and then partitions the graph to select execution devices for each operator. When an online request arrives, Chrion performs forward computation according to the graph partition by executing the operators on the CPU and GPU in parallel. Our experimental results show that the execution time can be reduced by 19.4% at most in the latency-optimal pattern and GPU memory footprint by 67.5% in the memory-optimal pattern compared with the execution on the GPU.

==> contents/4/4_2_algorithm_archive.tex <==
\subsection{Topological Sorting}

% explain the importance of sorting and existing drawbacks
%% importance
Given a computational graph, it is critial to determine the execution order for the vertices on the graph, which influences the inference efficiency on heterogeneous platforms and SLO satisfaction rate for users.
Depth-first-search (DFS) algorithm and breadth-first-search (BFS) algorithm are the two most commonly used graph traversal algorithms, which have been widely used in topological sorting.
%% BFS / DFS
Both starting from the root nodes, DFS explores feasible kernel functions as far as possible before backtracing, while BFS explores vertices by the order of their distances from the root nodes.
%% drawbacks
However, \fig{sorting-optim} demonstrates that simply applying BFS or DFS can not achieve ideal benefits. 
We assume there are two available devices and we always schedule the nodes according to the given order to a more idle device. 
It results in low parallelism if scheduling the kernel functions according to DFS, while high context switches between continuous kernels if according to BFS. 
The optimal situation should be that we can explore parallelism with BFS and maintain locality to reduce context switch with DFS.

%% inspirations

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\textwidth]{assets/topological-sorting-optim.pdf}
    \caption{Topological Sorting Optimization \zinuo{to be modified, not accurate}}
    \label{fig:sorting-optim}
\end{figure}

% our algorithm and optimization
Based on the observations above, we design a topological sorting method by taking advantage of BFS and DFS, and provide the pseudo code in Algorithm \ref{alg:sorting}.
%% function of bfs and dfs
We use BFS to expolore potential parallelism by distributing different branches to different devices for execution, and DFS to maintain locality by avoiding closely-related neighbour kernel functions being scheduled across devices.
%% algorithm description
In Algorithm \ref{alg:sorting}, we first initialize three variables, order $O$ to be returned by the algorithm, a ready queue $Q$ to store the those kernels that have no predcessors or whose kernels have been scheduled, and a mark list to record whether a kernel has been scheduled.
Different from the classical BFS algorithm, before appending the ready kernel $v_{curr}$ to $O$ (\zinuo{no. line}), we will check whether its child function can be merged.
If its child has only one predcessor and the communication time is larger than the average execution time among devices, it means maintaining the locality can achieve more benefits, and it is where DFS plays its role in the algorithm. 

\begin{algorithm}[!t]
    \caption{Topological Sorting}
    \label{alg:sorting}
    % custom keyword
    \SetKwData{In}{\textbf{in}}
    \SetKwData{To}{to}
    \DontPrintSemicolon
    \SetAlgoLined
    \KwIn {computational graph $G = (V, E)$}
    \KwOut {schedule order $O$}
      \Begin{
          initialize an empty order $O$ \;
          initialize an empty ready queue $Q$ \;
          initialize a mark list $marked \gets [false] \times n$ \;
          \For{$v_i$ in $V$}{
                \If{$\operatorname{pred}(v_i) = \varnothing$}{
                    push $v_i$ into $Q$ \;
                }
          }
          \While{$Q$ is not empty}{
              pop the first element $v_{curr}$ from $Q$
              % check whether all the parents are ready
              $ready = true$ \;
              $ready = ready \enspace  \&\& \enspace marked[v_j], v_j \in \operatorname{pred}(v_{curr})$ \;
              % if ready
              \eIf{$ready$}{
                  \zinuo{lack optimization part} \;
                  $marked[v_{curr}] = true$ \;
                  append $v_{curr}$ to $O$ \;
              }{
                push $v_{curr}$ into $Q$ \;
              }
          }
        \Return{$O$}
    }
\end{algorithm}

\subsection{Device Selection}

\begin{algorithm}[!t]
    \caption{Device Selection}
    \label{alg:selection}
    % custom keyword
    \SetKwData{In}{\textbf{in}}
    \SetKwData{To}{to}
    \DontPrintSemicolon
    \SetAlgoLined
    \KwIn {computational graph $G = (V, E)$, topological order $O$}
    \KwOut {device selection $S$, selected number of CPU cores $k^{*}$}
        \Begin{
        $\operatorname{TotalCosts} \gets []$ \;
        \For{$k^{\prime}$ in $[0, k]$}{
            $S_{k^{\prime}} \gets []$ \;
            $\operatorname{avail}[0, \cdots, k^{\prime}] \gets [0, \cdots, 0]$ \;
            \For{$i$ in $O$} {
                $\operatorname{Costs} \gets []$ \;
                \For{$j$ in $[0, k^{\prime}]$} {
                    compute $\operatorname{EST}(v_i, p_j)$ with Eq. \ref{equation:est} \;
                    compute $\operatorname{EFT}(v_i, p_j)$ with Eq. \ref{equation:eft} \;
                    compute $M(v_i, p_j)$ with Eq. \ref{equation:mem} \;
                    $\operatorname{cost}_j = \operatorname{EFT}(v_i, p_j) + \alpha{M(v_i, p_j)}$ \;
                    add $\operatorname{cost}_j$ to $\operatorname{Costs}$
                }
                set $S_{k^{\prime}}[i]$ to $j$ with the minimum $\operatorname{Costs}[j]$ \;
                update $L$ and $M$\;
            }
            add $(L + \alpha{M})$ to $\operatorname{TotalCosts}$ \;
        }
        select $k^{*}$ with the minimum $\operatorname{TotalCosts}[k^{*}]$ \;
        set device selection $S = S_{k^{*}}$ \;
        reduce data movements repeatedly \zinuo{not clear} \;
        \Return{$k^{*}$, $S$} \;
    }
\end{algorithm}

% introduction
The increasing number of model operators and variable hardware performance make it impractical to enumerate all the device selections to achieve the optimal. 
We design an adaptive algorithm to provide fine-grained device selection for each operator in the computational graph. 
The core idea of our algorithm is to use greedy method to select the appropriate device for each operator to perform the forward computation. 
After comparing the execution time of the operator with the available time of the hardware, the greedy algorithm always schedules the operator to the device that can let the operator end the execution earliest.

% initial implementation
We show the details of the device selection algorithm in Algorithm \ref{alg:selection}. 
The inputs of the adaptive device selection are the DAG and the topological order obtained by Algorithm \ref{alg:sorting} while its outputs are the optimal resource configuration and the device selection scheme for each operator.
% iterate over the number of cpu cores 
\name computes the cost for each kind of resource configuration. When the number of chosen CPU cores equals $k^\prime$, we first initialize the available time for each device (Line 5). 
Then we iterate over the topological order list to find the best device for each operator (Line 8-14).
For each operator $o_i$ in the order $O$, \name calculate the earliest finish time and memory requirement, and then decide which device to select to achieve the least cost.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.33\textwidth]{assets/device-selection-optim.pdf}
    \caption{Device Selection Optimization}
    \label{fig:device_selection}
\end{figure}

% further optimization
%% problem
However, experiments show that too many data movements between CPU and GPU lead to such severe contention in PCIe to communicate between heterogeneous platforms that restricted PCIe bandwidth becomes the bottleneck of hybrid execution.
%% solution
To reduce the requirements of data movements across devices, we identify several cases where unnecessary memory copies can be omitted without interference with execution time.
%% example
\fig{device_selection} illustrates three common selections that can be further optimized. The first two cases consider the device selection between parent nodes and child nodes. The device selection algorithm opts to keep the selection for parent node and child nodes to avoid multiple data movements when all child nodes or all the parent nodes are scheduled to a different device. The third case considers a linear branch with continuous operators scheduled across devices.
%% optimization
In Algorithm \ref{alg:selection}, \name will count the existence of the above cases that cause data movements and repeat eliminating tedious memory copy by optimizing the device selection until the number of data movements is less than a threshold. \zinuo{not clear}

